Non-linear Associative-Commutative Many-to-One Pattern Matching with Sequence Variables

Pattern matching is a powerful tool which is part of many functional programming languages as well as computer algebra systems such as Mathematica. Among the existing systems, Mathematica offers the most expressive pattern matching. Unfortunately, no open source alternative has comparable pattern matching capabilities. Notably, these features include support for associative and/or commutative function symbols and sequence variables. While those features have individually been subject of previous research, their comprehensive combination has not yet been investigated. Furthermore, in many applications, a fixed set of patterns is matched repeatedly against different subjects. This many-to-one matching can be sped up by exploiting similarities between patterns. Discrimination nets are the state-of-the-art solution for many-to-one matching. In this thesis, a generalized discrimination net which supports the full feature set is presented. All algorithms have been implemented as an open-source library for Python. In experiments on real world examples, significant speedups of many-to-one over one-to-one matching have been observed.

==> declaration.tex <==
% !TEX root = thesis.tex
%
%************************************************
% Declaration
%************************************************
\pdfbookmark[0]{Eidesstattliche Versicherung}{Eidesstattliche Versicherung}
\chapter*{Eidesstattliche Versicherung}
\label{sec:declaration}
\thispagestyle{empty}

Ich versichere hiermit an Eides Statt, dass ich die vorliegende Masterarbeit
selbstständig und ohne unzulässige fremde Hilfe erbracht habe. Ich habe keine anderen als
die angegebenen Quellen und Hilfsmittel benutzt.

\bigskip

\noindent\textit{\thesisUniversityCity, 24. April 2017}

\smallskip

\begin{flushright}
	\begin{minipage}{5cm}
		\rule{\textwidth}{1pt}
		\centering\thesisName
	\end{minipage}
\end{flushright}

%*****************************************
%*****************************************


==> title.tex <==

\pagestyle{empty}
%\setcounter{page}{0}

\begin{center}
{\Large Rheinisch-Westfälische Technische Hochschule Aachen\par}
		Aachen Institute for Advanced Study in Computational Engineering Science \\
		High-Performance and Automatic Computing Group
\vfill
{\large Master Thesis}
\vskip 2em
{\Huge\textsf{Non-linear Associative-Commutative Many-to-One Pattern Matching with Sequence Variables}\par}

%\vskip 3em
\vskip 1.5em
%{\large\textsf{
% Untertitel
%}\par}
\vskip 2.5em
{\large Manuel Krebber\par}
{\large Matrikelnr. 309878 \par}

\vskip -3em plus 2fill
{\large \today \par}
\vskip 5em

\begin{tabular}{ll}
	Betreuung:		& Prof. Paolo Bientinesi, Ph.D.\\
					& Henrik Bartels, M.Sc.\\
					& \\
	Zweitgutachter: & Dr. Diego Fabregat Traver
\\
\end{tabular}
\end{center}
\cleardoublepage
\vspace*{\fill}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Dieser Absatz muss exakt so in der Diplomarbiet enthalten sein und unterschrieben werden.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{}I hereby declare that I have created the work at hand completely on my own and
used no other sources or tools than the ones listed. Citations were marked accordingly.

\vspace{2cm}

\noindent{}Hiermit versichere ich, dass ich die Arbeit selbständig verfasst und keine anderen als die angegebenen Quellen und Hilfsmittel benutzt sowie Zitate kenntlich gemacht habe.

\vskip 3em

\noindent
Aachen, den \today
\vspace{2cm}

\cleardoublepage
\vfill


%\begin{center}
%{\Large\textbf{Danksagung}}\\
%\large
%\vskip 2cm
%An dieser Stelle könnte eine Danksagung stehen\\
%\vskip 1cm
%\noindent (an wen auch immer)\\
%\end{center}
%\vfill
%\cleardoublepage

